Multilingual Holistic Bias: Extending Descriptors and Patterns to Unveil Demographic Biases in Languages at Scale

We introduce a multilingual extension of the HOLISTICBIAS dataset, the largest English template-based taxonomy of textual people references: MULTILINGUALHOLISTICBIAS. This extension consists of 20,459 sentences in 50 languages distributed across all 13 demographic axes. Source sentences are built from combinations of 118 demographic descriptors and three patterns, excluding nonsensical combinations. Multilingual translations include alternatives for gendered languages that cover gendered translations when there is ambiguity in English. Our benchmark is intended to uncover demographic imbalances and be the tool to quantify mitigations towards them. Our initial findings show that translation quality for EN-to-XX translations is an average of 8 spBLEU better when evaluating with the masculine human reference compared to feminine. In the opposite direction, XX-to-EN, we compare the robustness of the model when the source input only differs in gender (masculine or feminine) and masculine translations are an average of almost 4 spBLEU better than feminine. When embedding sentences to a joint multilingual sentence representations space, we find that for most languages masculine translations are significantly closer to the English neutral sentences when embedded.

==> figures/contributions.tex <==


\definecolor{color0}{HTML}{FFFFFF}
\definecolor{color1}{HTML}{FFEDE5}
\definecolor{color2}{HTML}{FEE5D8}
\definecolor{color3}{HTML}{FED9C9}
\definecolor{color4}{HTML}{FDCAB5}
\definecolor{color5}{HTML}{FCBBA1}




\newcommand*{\mybox}[2]{{\setlength{\fboxsep}{0.15pt}\colorbox{#1}{\strut #2}}}


%\newcommand*{\mybox}[2]{\tikz[anchor=base,baseline=0pt,rounded corners=0pt, inner sep=0.2mm] %\node[fill=#1!60!white] (X) {#2};}
%\newcommand*{\mybbox}[2]{\tikz[anchor=base,baseline=0pt,inner sep=0.2mm,] %\node[draw=black,thick,fill=#1!60!white] (X) {#2};}

\begin{figure*}[width=\textwidth]
\centering
\begin{tabular}{@{}p{13.5cm}@{\hspace{0.2cm}}p{13.5cm}@{}}
%  \resizebox{0.49\textwidth}{!}{%
  \small 
 \textbf{Hallucination}\\
 \midrule
 \small Sentence 1 \\ 
 \small
 \mybox{color0}{\strut{$\_$$\_$eng$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{I}} \mybox{color0}{\strut{love}} \mybox{color0}{\strut{being}} \mybox{color4}{\strut{chubby.}} \mybox{color0}{\strut{$<$/s$>$}}  \mybox{color0}{\strut{$<$/s$>$}} \mybox{color1}{\strut{$\_$$\_$fra$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{J'adore}} \mybox{color0}{\strut{être}} \mybox{color2}{\strut{une}} \mybox{color5}{\strut{grosse}} \mybox{color0}{\strut{\bf{chatte}.}}\\ %part8 unfiltered 9564
  \midrule
  \small 
 \textbf{Mistranslation}\\
 \midrule
 \small Sentence 2 \\
 \midrule
 \small
 \mybox{color0}{\strut{$\_$$\_$eng$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{Hi!}} \mybox{color0}{\strut{I'm}} \mybox{color0}{\strut{a}} \mybox{color5}{\strut{gangly}} \mybox{color1}{\strut{child.}} \mybox{color0}{\strut{$<$/s$>$}} \mybox{color0}{\strut{$<$/s$>$}} \mybox{color4}{\strut{$\_$$\_$cat$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{Hola,}} \mybox{color0}{\strut{sóc}} \mybox{color0}{\strut{un}} \mybox{color4}{\strut{nen}} \mybox{color0}{\strut{\bf{malparit}.}}\\
  \midrule
  \small
%\textbf{Semantically related translation, wrong level of offensiveness}\\
%\midrule
% \small Sentence 3 \\
% \midrule
% \small
% \mybox{color0}{\strut{$\_$$\_$eng$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{Hi}} \mybox{color0}{\strut{I'm}} \mybox{color0}{\strut{a}} \mybox{color5}{\strut{queer}} \mybox{color2}{\strut{sibling.}} \mybox{color0}{\strut{$<$/s$>$}} \mybox{color0}{\strut{$<$/s$>$}} \mybox{color1}{\strut{$\_$$\_$spa$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{Hola}} \mybox{color0}{\strut{soy}} \mybox{color0}{\strut{un}} \mybox{color2}{\strut{hermano}} \mybox{color0}{\strut{\bf{marica}.}}\\
%\mybox{color0}{\strut{$\_$$\_$eng$\_$Latn$\_$$\_$}} %\mybox{color0}{\strut{I'm}} \mybox{color0}{\strut{not}} %\mybox{color0}{\strut{a}} \mybox{color5}{\strut{queer}} %\mybox{color1}{\strut{guy.}} \mybox{color0}{\strut{$<$/s$>$}} %\mybox{color0}{\strut{$<$/s$>$}} %\mybox{color3}{\strut{$\_$$\_$cat$\_$Latn$\_$$\_$}} %\mybox{color0}{\strut{No}} \mybox{color0}{\strut{sóc}} %\mybox{color0}{\strut{un}} \mybox{color2}{\strut{tipus}} %\mybox{color0}{\strut{\bf{maricona}.}}\\
% \midrule
% \small
 %\textbf{Semantically related translation, correct level of offensiveness}\\
 \textbf{Correct translation}\\
\midrule
 \small Sentence 3 \\
 \midrule
 \small
%  \mybox{color0}{\strut{$\_$$\_$eng$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{Hi!}} \mybox{color0}{\strut{I'm}} \mybox{color0}{\strut{a}} \mybox{color0}{\strut{person}} \mybox{color0}{\strut{with}} \mybox{color5}{\strut{dyslexia.}} \mybox{color0}{\strut{</s>}} \mybox{color0}{\strut{</s>}} \mybox{color2}{\strut{$\_$$\_$cat$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{Hola!}} \mybox{color0}{\strut{Sóc}} \mybox{color0}{\strut{una}} \mybox{color0}{\strut{persona}} \mybox{color3}{\strut{amb}} \mybox{color0}{\strut{dislèxia.}}\\
   \mybox{color0}{\strut{$\_$$\_$eng$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{Hi!}} \mybox{color1}{\strut{I'm}} \mybox{color0}{\strut{a}} \mybox{color5}{\strut{50-year-old}} \mybox{color1}{\strut{woman.}} \mybox{color0}{\strut{$<$/s$>$}} \mybox{color0}{\strut{$<$/s$>$}} \mybox{color3}{\strut{$\_$$\_$cat$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{Hola,}} \mybox{color0}{\strut{sóc}} \mybox{color0}{\strut{una}} \mybox{color3}{\strut{dona}} \mybox{color0}{\strut{de}} \mybox{color0}{\strut{\bf{50}}} \mybox{color0}{\strut{\bf{anys}.}}\\
\midrule

  \end{tabular}
  \caption{Examples of translations in English-to-French, English-to-Spanish or English-to-Catalan.
  %Each sentence shows the input attribution to the word in bold  
  Sentences show input attributions for bold words in the cases of hallucination (sentence 1); mistranslation (sentence 2); %a semantically related translation but wrong level of offensiveness (sentence 3); 
  and a correct translation (sentence 3).  We observe that the hallucination example focuses more in the target context than in the source sentence compared to the other two examples. \label{fig:hallucinationmistranslation}}
\end{figure*}


==> tables/results7languages.tex <==
\begin{table*}[h]
\large
\centering
    \begin{tabular}{clrrrrrrr} 
    \toprule
    & & \multicolumn{4}{c}{\textbf{Holistic Bias}} & \multicolumn{3}{c}{\textbf{FLORES 200}}  \\
    \cmidrule(lr){3-6} 	\cmidrule(lr){7-9}
    Language & Model & \multicolumn{2}{c}{Detoxify} & ETOX & LaBSE & BLEU & CHRF &  TER \\ 
     & & Score & $\abs{\bigtriangleup}$ & & & &&\\ 

            \midrule
            	spa\_Latn&Baseline&0.9&0.69&981&0.85&20.39&46.57&64.45\\

            	&ETOX&0.36&0.34&314&0.82&20.33&46.53&64.54\\
		          &Detoxify&0.22&0.25&168&0.81&20.22*&46.51&64.63\\
            \midrule
            	tur\_Latn&Baseline&0.93&0.64&299&0.82&19.39&49.7&66.29\\

            	&ETOX&0.5&0.36&67&0.78&19.27&49.62&66.4\\
		          &Detoxify&0.44&0.35&63&0.76&18.86*&49.47&66.8*\\
            \midrule
            	por\_Latn&Baseline&0.48&0.38&1471&0.85&35.99&58.48&49.69\\

            	&ETOX&0.17&0.18&911&0.81&35.84*&58.36*&49.85*\\
		          &Detoxify&0.14&0.17&877&0.82&35.63*&58.26*&50.02*\\
            \midrule
            	ita\_Latn&Baseline&0.92&0.77&821&0.86&20.77&47.99&64.85\\

            	&ETOX&0.29&0.27&197&0.82&20.71&48.03&65.01\\
		          &Detoxify&0.21&0.22&135&0.81&20.63&47.96&65.08*\\
            \midrule
            	fra\_Latn&Baseline&0.9&0.75&418&0.79&32.73&54.82&53.82\\

            	&ETOX&0.33&0.32&106&0.78&32.32*&54.55*&54.25*\\
		          &Detoxify&0.2&0.25&71&0.77&32.43*&54.71&54.21*\\
            \midrule
            	rus\_Cyrl&Baseline&0.85&0.66&151&0.84&19.61&44.91&68.25\\

            	&ETOX&0.42&0.39&60&0.77&19.61&44.94&68.25\\
		          &Detoxify&0.26&0.29&38&0.75&19.48&44.95&68.53\\
    \bottomrule
    \end{tabular}%
  \caption{Results for 6 languages: for holistic bias in terms of toxicity (detoxify and ETOX) and translation quality (LaBSE); and for FLORES in terms of translation quality (BLEU, chrF and TER). ($*$) means difference statistically significant.}
  \label{tab:results7languages}
\end{table*}
